Estimating Functionals of the Joint Distribution of Potential Outcomes with Optimal Transport

Many causal parameters depend on a moment of the joint distribution of potential outcomes. Such parameters are especially relevant in policy evaluation settings, where noncompliance is common and accommodated through the model of Imbens & Angrist (1994). This paper shows that the sharp identified set for these parameters is an interval with endpoints characterized by the value of optimal transport problems. Sample analogue estimators are proposed based on the dual problem of optimal transport. These estimators are root-n consistent and converge in distribution under mild assumptions. Inference procedures based on the bootstrap are straightforward and computationally convenient. The ideas and estimators are demonstrated in an application revisiting the National Supported Work Demonstration job training program. I find suggestive evidence that workers who would see below average earnings without treatment tend to see above average benefits from treatment.

==> sections/OTJointPO_section_simulations.tex <==
\section{Simulations}
\label{Section: simulations}

\begin{mdframed}
	\begin{center}
		[Some nice simulations]
	\end{center}
\end{mdframed}

